Sampling-based Continuous Optimization with Coupled Variables for RNA Design

The task of RNA design given a target structure aims to find a sequence that can fold into that structure. It is a computationally hard problem where some version(s) have been proven to be NP-hard. As a result, heuristic methods such as local search have been popular for this task, but by only exploring a fixed number of candidates. They can not keep up with the exponential growth of the design space, and often perform poorly on longer and harder-to-design structures. We instead formulate these discrete problems as continuous optimization, which starts with a distribution over all possible candidate sequences, and uses gradient descent to improve the expectation of an objective function. We define novel distributions based on coupled variables to rule out invalid sequences given the target structure and to model the correlation between nucleotides. To make it universally applicable to any objective function, we use sampling to approximate the expected objective function, to estimate the gradient, and to select the final candidate. Compared to the state-of-the-art methods, our work consistently outperforms them in key metrics such as Boltzmann probability, ensemble defect, and energy gap, especially on long and hard-to-design puzzles in the Eterna100 benchmark. Our code is available at: http://github.com/weiyutang1010/ncrna_design.

==> related.old.tex <==
% !TEX root = main.tex

\section{Related Work}

The recent work by \namecite{matthies+:2023}
proposes a framework very similar to our expected partition function, which they call the ``structure-sequence partition function'',
but from a  different motivation
and for the different
%continuous optimization 
task %(which they call ``differentiable partition function'')
%
of non-coding (ncRNA) RNA design.
%The major difference is that our work presents a general framework that applies to both mRNA design and ncRNA design.
%%\footnote{The formulation of expected partition function and preliminary results on mRNA design were included in an NIH proposal 1 R01 GM151529-01 by the corresponding author (submitted Oct.~2022).}.
They first defined the concept of  ``sequence partition function'' as $$\expQy (\distri) = \sum_{\vecx} \distri(\vecx) e^{-\Delta G(\vecx,\vecy) / RT} =  \E_{\vecx \sim \distri(\cdot)}[e^{-\Delta G(\vecx, \vecy) / RT}] ,$$ 
and then extended it to the ``structure-sequence partition function'': 
$$\expQ (\distri) =  \sum_{\vecy}  \expQy (\distri) .$$ 

We argue that this framework is a better fit for mRNA design than ncRNA design because as \namecite{zhang+:2023} showed,
the mRNA design space can be categorized by a regular language (or finite-state automata) and the objective function (either MFE or partition function) can be formulated as a stochastic context-free grammar (SCFG).
It is well-known in formal language theory that the intersection of a (stochastic) context-free language and a regular language is another (stochastic)  context-free language, which is the essential reason why 
\namecite{zhang+:2023}'s algorithm for MFE-based mRNA design 
runs in worst-case $O(n^3)$ time.
By contrast, the design space for ncRNA design given a target structure \vecy is not a regular, but rather a context-free language, because
the paired positions in \vecy are correlated
(for any pair $(i,j)\in \vecy$, $x_i x_j$ must be pairable; it is straightforward to write a context-free grammar for the set of 
all possible \vecx for $\vecy$). 
Unfortunately, the intersection of two context-free languages are context sensitive, which rules out polynomial-time algorithms. This observation suggests that ncRNA design is fundamentally harder than mRNA design, and this framework is more promising for mRNA design.


%Even for ncRNA design problem that both work attempted to solve, there is a critical difference in the objective function formulation, which we detail in the Appendix~\ref{sec:appendix_ours_vs_maxs}. 
%In terms of implementation for ncRNA design, theirs is in Python and in the original space (i.e., $(+,\times)$ semiring) which will inevitably suffer from overflowing/underflowing on longer structures, while ours is in C++ (based on the LinearPartition codebase) and in logspace (i.e., $(\oplus_{\log}, +)$ semiring) which has the potential of better scalability.


